Impact of pions on binary neutron star mergers

We study the impact of pions in simulations of neutron star mergers and explore the impact on gravitational-wave observables. We model charged and neutral pions as a non-interacting Boson gas with a chosen, constant effective mass. We add the contributions of pions, which can occur as a condensate or as a thermal population, to existing temperature and composition dependent equations of state. Compared to the models without pions, the presence of a pion condensate decreases the characteristic properties of cold, non-rotating neutron stars such as the maximum mass, the radius and the tidal deformability. We conduct relativistic hydrodynamical simulations of neutron star mergers for these modified equations of state models and compare to the original models, which ignore pions. Generally, the inclusion of pions leads to a softening of the equation of state, which is more pronounced for smaller effective pion masses. We find a shift of the dominant postmerger gravitational-wave frequency by up to 150~Hz to higher frequencies and a reduction of the threshold binary mass for prompt black-hole formation by up to 0.07~$M_\odot$. We evaluate empirical relations between the threshold mass or the dominant postmerger gravitational-wave frequency and stellar parameters of nonrotating neutron stars. These relations are constructed to extract these stellar properties from merger observations and are built based on large sets of equation of state models which do not include pions. Comparing to our calculations with pions, we find that these empirical relations remain valid to good accuracy, which justifies their use although they neglect a possible impact of pions. We also address the mass ejection by neutron star mergers and observe a moderate enhancement of the ejecta mass by a few ten per cent. (abridged)

==> journalheader.tex <==
\newcommand{\apjl}{Astrophys. J. Lett.}%
          % Astrophysical Journal, Letters
\newcommand{\apjs}{Astrophys. J. Supp.}%
          % Astrophysical Journal, Letters
\newcommand{\aap}{Astron. Astrophys.}%
          % Astrophysical Journal, Letters    
\newcommand{\mnras}{Mon. Not. Roy. Astron. Soc.}%
          % Astrophysical Journal, Letters   
\newcommand{\lrr}{Living Reviews in Relativity}%
          % Living reviews         
\newcommand{\pasa}{Publications of the Astronomical Society of Australia}
          %Publications of the Astronomical Society of Australia
          
          

